AI and Collective Decisions: Strengthening Legitimacy and Losers' Consent

AI is increasingly used to scale collective decision-making, but far less attention has been paid to how such systems can support procedural legitimacy, particularly the conditions shaping losers' consent: whether participants who do not get their preferred outcome still accept it as fair. We ask: (1) how can AI help ground collective decisions in participants' different experiences and beliefs, and (2) whether exposure to these experiences can increase trust, understanding, and social cohesion even when people disagree with the outcome. We built a system that uses a semi-structured AI interviewer to elicit personal experiences on policy topics and an interactive visualization that displays predicted policy support alongside those voiced experiences. In a randomized experiment (n = 181), interacting with the visualization increased perceived legitimacy, trust in outcomes, and understanding of others' perspectives, even though all participants encountered decisions that went against their stated preferences. Our hope is that the design and evaluation of this tool spurs future researchers to focus on how AI can help not only achieve scale and efficiency in democratic processes, but also increase trust and connection between participants.

==> tables/concept_explanations_table.tex <==
\begin{table}[ht]
\footnotesize
\centering
\begin{tabular}{>{\raggedright\arraybackslash}p{0.1\linewidth}>{\raggedright\arraybackslash}p{0.15\linewidth}p{0.7\linewidth}}
\toprule
Domain & Concept & Description \\
\midrule
\multirow{4}{*}{Process Legitimacy} 
  & Understood Decisions & Did the participant understand how the decisions were made? \\
  & Trust & Did the participant trust the decisions accurately reflected the participants' views? \\
  & Adherence & Would the participant be willing to abide by the decisions? \\
  & Felt Heard & Did the participant feel their input was valuable? \\
\midrule
\multirow{11}{*}{Social Cohesion} 
  & Learning about others & Did the participant understand others' beliefs and experiences? \\
  & Feel Connected & How connected did the participant feel to others? \\
  & Respect & Did the participant respect others' beliefs and views? \\
  & Rational & Did the participant feel others were rational? \\
  & Inclusion of Self in Others  & A visual scale that estimates how close participants feel to others. \\
  & Perspective-taking & Could the participant understand how others may view the proposals? \\
  & Commonalities & Did the participant have commonalities with other participants? \\
  & Respect Pluralism & Did the participant think it's important to respect a diversity of views? \\
  & Curious About Others  & How curious was the participant about others? \\
  & Willing to Interact & Would the participant be willing to interact with others? \\
\midrule
\multirow{4}{*}{Stances and Learning} 
  & Learning about topics & Did the participant learn more about the topics? \\
  & Change stance & Did the participant report that their stance had shifted? \\
  & Topic stance & How much did the participant agree with the proposal? \\
  & Stance certainty & How certain was the participant in their stance? \\
\bottomrule
\end{tabular}
\caption{We show the hierarchy of our measurement framework here with a short description of each concept.}
\label{tab:domain_conc}
\end{table}


==> tables/domains_concepts_items_simplified.tex <==
\begin{table}[ht]
\centering
\footnotesize
\begin{tabular}{|p{4cm}|p{5cm}|p{8cm}|}
\hline
\textbf{Domains} & \textbf{Concepts} & \textbf{Items} \\
\hline
\multirow{15}{4cm}{Process Legitimacy} & \multirow{3}{5cm}{Trust} & I trust the legitimacy of the votes that came of this process. \\
 &  & informed. \\
 &  & I would be hesitant to rely this process to make and vote on proposals on other issues. \\
 & \multirow{3}{5cm}{Felt Heard} & I felt that my input was valuable in this process. \\
 &  & My own opinions and experiences were not reflected in any way by the proposals. \\
 &  & I felt heard during this process. \\
 & \multirow{4}{5cm}{Understood Decisions} & I understood how the proposal decisions were made. \\
 &  & I had a strong understanding of how participants’ opinions and experiences informed the decisions on the proposals. \\
 &  & I was unsure how participants’ opinions and experiences aligned with or diverged from each proposal. \\
 &  & I understood why each proposal decision was made. \\
 & \multirow{5}{5cm}{Adherence} & I would be willing to abide by the specific proposal decisions generated from this process. \\
 &  & Generally, I would be willing to abide by proposal decisions from this process (on other issues). \\
 &  & Even if I disagreed with certain proposal decisions, I would view them as being legitimately created. \\
 &  & Even if I disagreed with certain proposal decisions, I would still respect them. \\
 &  & Even if I disagreed with certain proposal decisions, I would still adhere to them. \\
\hline
\multirow{28}{4cm}{Social Cohesion} & \multirow{1}{5cm}{Inclusion of Self in Others} & Think about yourself (Self) and the other participants in this study (Other). In this exercise, we are interested in how similar you see yourself and the other participants. If you see yourself and the other participants as very similar, you would choose circles that overlap more so with each other. If you see yourself and other participants as less similar, you would choose circles that overlap less so with each other. Please choose which picture best shows the relationship between you and the other participants in this study. \\
 & \multirow{1}{5cm}{Feel Connected} & I feel connected to the other participants whose interviews were used to generate these proposals. \\
 & \multirow{1}{5cm}{Willing to Interact} & I would be willing to interact with the other participants whose interviews helped to generate the proposals. \\
 & \multirow{1}{5cm}{Curious About Others} & I don’t feel a desire to learn more about the other participants whose interviews helped generate the proposals. \\
 & \multirow{3}{5cm}{Rational} & Are irrational for holding their stances on this topic \\
 &  & Have a stance that makes sense \\
 &  & Are logical for holding their stance \\
 & \multirow{5}{5cm}{Respect} & I have respect for the other people whose experiences and opinions helped create these proposals. \\
 &  & Even if I were disagreed with proposal decisions generated by this process, I still have respect for the people that support it. \\
 &  & Disregard the other participants’ points of view \\
 &  & Be considerate of the other participants’ stances \\
 &  & Take the other participants’ points of view \\
 & \multirow{4}{5cm}{e} & I probably have things in common with the other participants whose experiences and opinions helped to create these proposals. \\
 &  & I probably share values, opinions, or experiences with others who were part of this process. \\
 &  & I probably have very little in common with other people who were part of this process. \\
 &  & I am reading all of the questions in this survey carefully. \\
 & \multirow{3}{5cm}{Perspective-taking} & I feel confident in predicting why different people might support or oppose a given proposal. \\
 &  & I feel confident in identifying the key pros and cons of a given proposal. \\
 &  & I would struggle to understand how someone with a different background or values might view each proposal. \\
 & \multirow{4}{5cm}{Learn about others} & I learned more about others’ experiences and opinions on this topic by interacting with the proposals. \\
 &  & I understood other participants more holistically by interacting with the proposals. \\
 &  & I was able to understand why other participants have certain beliefs or opinions on the topic. \\
 &  & This process did not clarify participants’ experiences, beliefs, or opinions for me. \\
 & \multirow{5}{5cm}{Respect Pluralism} & I find it difficult to be open to political views that differ from my own. \\
 &  & I respect people who disagree with me on political issues. \\
 &  & I would be willing to interact with someone who disagrees with me on political issues. \\
 &  & It is important for people to respect a diversity of different opinions. \\
 &  & If someone disagrees with me on a political issue, they probably have a good reason for doing so. \\
\hline
\multirow{24}{4cm}{Stances and Learning} & \multirow{9}{5cm}{Learning about topics} & Compared to before, I feel more informed about why people may have different beliefs on raising the minimum wage. \\
 &  & I feel more informed about the topic of raising the minimum wage. \\
 &  & This exercise has taught me something about raising the minimum wage. \\
 &  & Compared to before, I feel more informed about why people may have different beliefs on hiring locals over international applicants. \\
 &  & I feel more informed about the topic of hiring locals over international applicants \\
 &  & This exercise has taught me something about the topic of hiring locals over international applicants. \\
 &  & Compared to before, I feel more informed about why people may have different beliefs about the topic of using race and gender in hiring. \\
 &  & I feel more informed about the topic of using race and gender in hiring decisions. \\
 &  & This exercise has taught me something about the topic of using race and gender in hiring decisions. \\
 & \multirow{9}{5cm}{Stance certainty} & I hold strong beliefs about whether the federal minimum wage should be raised. \\
 &  & I feel certain that my stance on the federal minimum wage is the right one. \\
 &  & I don't think there are good arguments against my position on whether to raise the federal minimum wage. \\
 &  & I hold strong beliefs about whether companies should prioritize locals over international applicants. \\
 &  & I feel certain that my stance on whether companies should prioritize local applicants over international ones is the right one. \\
 &  & I don't think there are good arguments against my position on whether to prioritize locals over international applicants. \\
 &  & I hold strong beliefs about whether race and gender should be used in hiring decisions. \\
 &  & I feel certain that I hold the correct belief on whether race and gender should be used in hiring decisions. \\
 &  & I don't think there are good arguments against my position on whether race and gender should be used in hiring decisions. \\
 & \multirow{3}{5cm}{Change stance (self report)} & Compared to before this process, my beliefs on the minimum wage issue have: \\
 &  & Compared to before this process, my beliefs on hiring international applicants has: \\
 &  & Compared to before this process, my beliefs on whether race or gender should be used in hiring decisions have: \\
 & \multirow{3}{5cm}{Topic stance} & How much do you agree with the following statement? 

"The federal minimum wage should be raised to \$30 an hour." \\
 &  How much do you agree with the following statement?



"Companies should strongly prioritize hiring domestically before considering foreign applicants." \\
 &  & How much do you agree with the following statement?



"Race and gender should be used in hiring decisions to combat inequality in the workplace." \\
\hline
\end{tabular}
\caption{Domains, Concepts, and Items with Simplified Clean Names}
\end{table}

==> tables/featured_prof.tex <==
\begin{table}[ht]
\centering
% \begin{tabular}{p{10cm}ccc}
\begin{tabularx}{\columnwidth}{@{}Xcc@{}}
\toprule
\textbf{Statement} & \textbf{Low (0--33)} & \textbf{Mid (33--66)} & \textbf{High (66+)} \\
\midrule
The federal minimum wage should be raised to \$30 an hour. & 5  & 10 & 23 \\
Companies should strongly prioritize hiring domestically before considering foreign applicants. & 7  & 4  & 8  \\
Race and gender should be used in hiring decisions to combat inequality in the workplace. & 17 & 9  & 8  \\
\bottomrule
\end{tabularx}
\caption{Responses categorized by support levels for different policy statements.}
\label{tab:policy_responses}
\end{table}


==> tables/process_table.tex <==
\begin{table}[H]
\caption{Outcomes associated with adherence to participatory processes across visualization and interview modes.}
\centering
\footnotesize
\begin{tabular}{p{2cm}p{4cm}cccccccc}

\toprule
\multicolumn{2}{c}{} & \multicolumn{4}{c}{\textbf{Visualization}} & \multicolumn{4}{c}{\textbf{Interview}} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10}
\textbf{Category} & \textbf{Outcome} & Coef. & 90\% CI & pval & qval & Coef. & 90\% CI & pval & qval \\
\midrule
\multirow{5}{*}{Adherence} & \textbf{I would be willing to abide by the specific proposal decisions generated from this process.} & 0.88* & [0.26, 1.49] & 0.02 & 0.10 & 0.43 & [-0.20, 1.06] & 0.26 & 0.81 \\
 & Generally, I would be willing to abide by proposal decisions from this process (on other issues). & 0.64 & [0.01, 1.26] & 0.09 & 0.12 & 0.38 & [-0.26, 1.03] & 0.32 & 0.81 \\
 & Even if I disagreed with certain proposal decisions, I would view them as being legitimately created. & 0.69 & [0.08, 1.29] & 0.06 & 0.12 & 0.04 & [-0.58, 0.66] & 0.92 & 0.93 \\
 & Even if I disagreed with certain proposal decisions, I would still respect them. & 0.60 & [0.03, 1.17] & 0.08 & 0.12 & 0.03 & [-0.55, 0.62] & 0.93 & 0.93 \\
 & Even if I disagreed with certain proposal decisions, I would still adhere to them. & 0.14 & [-0.44, 0.72] & 0.69 & 0.69 & 0.10 & [-0.50, 0.70] & 0.78 & 0.93 \\
\multirow{3}{*}{Felt Heard} & \textbf{I felt that my input was valuable in this process.} & 0.98** & [0.39, 1.57] & 0.01 & 0.02 & 0.63 & [0.03, 1.23] & 0.09 & 0.13 \\
 & My own opinions and experiences were not reflected in any way by the proposals. & 0.42 & [-0.27, 1.11] & 0.32 & 0.48 & -0.04 & [-0.75, 0.67] & 0.93 & 0.93 \\
 & \textbf{I felt heard during this process.} & 0.11 & [-0.36, 0.59] & 0.70 & 0.70 & 1.99*** & [1.50, 2.48] & 0.00 & 0.00 \\
\multirow{3}{*}{Trust \& Legitimacy} & \textbf{I trust the legitimacy of the votes that came of this process.} & 1.47*** & [0.88, 2.07] & 0.00 & 0.00 & 0.58 & [-0.03, 1.18] & 0.12 & 0.36 \\
 & \textbf{I think the votes on these proposals were well-informed.} & 1.24*** & [0.60, 1.87] & 0.00 & 0.00 & 0.37 & [-0.29, 1.02] & 0.35 & 0.53 \\
 & \textbf{I would be hesitant to rely this process to make and vote on proposals on other issues.} & 0.93** & [0.26, 1.60] & 0.02 & 0.02 & 0.03 & [-0.66, 0.71] & 0.95 & 0.95 \\
\multirow{4}{*}{Understood Decisions} & \textbf{I understood how the proposal decisions were made.} & 1.11*** & [0.49, 1.73] & 0.00 & 0.00 & 0.38 & [-0.25, 1.02] & 0.32 & 0.42 \\
 & \textbf{I had a strong understanding of how participants’ opinions and experiences informed the decisions on the proposals.} & 1.55*** & [0.93, 2.16] & 0.00 & 0.00 & 0.61 & [-0.02, 1.24] & 0.11 & 0.42 \\
 & \textbf{I was unsure how participants’ opinions and experiences aligned with or diverged from each proposal.} & 1.55*** & [0.87, 2.23] & 0.00 & 0.00 & -0.11 & [-0.81, 0.59] & 0.79 & 0.79 \\
 & \textbf{I understood why each proposal decision was made.} & 1.24*** & [0.64, 1.83] & 0.00 & 0.00 & 0.41 & [-0.20, 1.02] & 0.27 & 0.42 \\
\bottomrule
\end{tabular}

\end{table}


==> tables/questions_longtable.tex <==
% Requires: \usepackage{longtable} and \usepackage{booktabs}
\setlength{\LTpre}{0pt}\setlength{\LTpost}{0pt}
\begin{center}
\footnotesize
\vspace{0.5em}
\begin{longtable}{p{7cm} p{7cm} r}
\toprule
\textbf{Question} & \textbf{Instruction} & \textbf{Max Sec} \\
\midrule
\endfirsthead
\toprule
\textbf{Question} & \textbf{Instruction} & \textbf{Max Sec} \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{\emph{Continued on next page}}\\
\endfoot
\bottomrule
\endlastfoot
To start off, can you tell me a bit about your background? Where did you grow up, and what was it like? You can share anything about your family, your neighborhood, friends, or anything else you can think of. & Learn as much as you can about the interviewee's life experience, and their personal background. Be respectful but curious as you hear about their story. Try to get some specific and detailed experiences or memories about the interviewee's life. & 30 \\
Now I'd like to ask you about an important relationship in your life. Who is someone who has had a big impact on you? Can you tell me about your relationship with them—how you met, what they mean to you, and any important memories you've shared? & Learn about a personally meaningful relationship. Encourage storytelling and emotional depth. Ask follow-ups to explore how this relationship shaped the interviewee's identity, values, or perspective. & 30 \\
Can you tell me about the work you do now? What's your job like, and how do you feel about it day to day? & Learn about what the interviewee does for a living. Be curious but respectful as you hear about their story. Follow up and ask what they like and dislike about their job. & 45 \\
Generally, what could be done to make your work life better? You can discuss whatever you feel would make your life better, either now or in the past. & Learn about what the interviewee thinks could be done to make their work life better. Be curious about their thoughts. Try to get some specific examples or ideas about how to improve their work life. If they need inspiration, you can give them some ideas but try not to bias them. If their answers are too brief or surface-level, probe further to understand their reasoning. You can even ask them what they would tell someone in-power like a lawmaker or employer. & 60 \\
We're now going to turn to the topic of the minimum wage. How would changes in the minimum wage (either raising or lowering it) affect you, your family, or anyone else you know personally? & Learn about how the interviewee thinks changes in the minimum wage would affect them, their family, or anyone else they know personally. Be curious about their thoughts. Make sure you ask follow up questions to get more specific on how they would be impacted. If they say they would be negatively impacted, ask why they think that. If they do not think they would be impacted, prompt them to think about different people they interact with that may be impacted. & 60 \\
What do you think is a fair minimum wage in your area? Why? & Understand the interviewee's thoughts on what a fair minimum wage is. Be curious and try to get some specific and detailed thoughts about the interviewee's thoughts on what a fair minimum wage is. For example, you can ask them to think about rent, food, and other basic necessities in their area. & 45 \\
If you earned more, what would you do with the extra money? & Learn about how the interviewee would spend extra money. You can also ask how it would make them feel to have the extra money, and what goals it would allow them to achieve. & 45 \\
Do you have any concerns about raising the minimum wage to \$30 an hour? & Surface how the interviewee thinks about economic trade-offs and competing narratives. If they cannot think of any downsides, you can provide some examples, such as higher prices, less jobs, etc. & 45 \\
I'd now like to ask you about discrimination. Have you ever experienced discrimination? If so, can you tell me about it? & Learn about the interviewee's experiences with discrimination. Be curious and try to get some specific and detailed experiences or memories about the interviewee's experience with discrimination. Follow up with questions about whether they have experienced discrimination in the workplace or hiring. If they say they have never experienced discrimination, ask them if anyone they know has experienced discrimination. If they say they have not experienced discrimination nor have anyone they know has experienced discrimination, then ask them whether they think discrimination is a problem in society and why. & 60 \\
How would you feel if you knew that race or gender was a factor in a hiring decision that affected you? & Understand the interviewee's thoughts on how they would feel if they knew that race or gender was a factor in hiring decisions. Be curious and try to get some specific and detailed thoughts about the interviewee's thoughts on how they would feel if they knew that race or gender was a factor in hiring decisions. & 45 \\
Do you think race or gender should be taken into account for hiring decisions to combat gender and racial inequality? Why or why not? & Understand the interviewee's thoughts on whether race or gender should be taken into account for hiring decisions. Be curious and try to get some specific and detailed thoughts about the interviewee's thoughts on whether race or gender should be taken into account for hiring decisions. & 45 \\
We're now going to move to a new topic. Have you ever worked with or known someone at work from another country? What was your experience like? & Understand whether the interviewee has worked with or known someone from another country. If they have, ask them specifics questions about their experience working with them and what it was like. If they have not, ask them if they have friends or family who are from another country, or they themselves are from another country. If they know someone from another country, ask them about that relationship and what it was like. & 45 \\
Have you or someone close to you ever been impacted by immigration policy, especially around work or hiring? & Understand whether the interviewee has been impacted by immigration policy. If they have, ask them specifics questions about their experience and what it was like. If they have not, ask them if they have friends or family who have been impacted by immigration policy. Try to get specific experiences or memories about the interviewee's experience with immigration policy if they have been impacted. If they have not been impacted at all nor have anyone they know has been impacted, then the objective has been met. & 45 \\
Do you think it matters where someone is from when hiring for a job, as long as they’re qualified? Why or why not? & Understand the interviewee's thoughts on whether it matters where someone is from when hiring for a job, as long as they’re qualified. Try to understand the benefits and drawbacks they see. Also follow up by asking if there are any situations where nationality or immigration status should be considered. & 45 \\
How do you feel about the idea that companies should prioritize hiring local applicants over foreign applicants? & Understand the interviewee's thoughts on the idea that companies should prioritize hiring local applicants over foreign applicants. Follow up by asking them the benefits and drawbacks of this idea. & 45 \\
\end{longtable}
\captionof{table}{Interview Questions with Instructions and Maximum Time}
\label{tab:questions_long}
\end{center}


==> tables/questions_table.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{|p{7cm}|p{7cm}|c|}
\hline
\textbf{Content} & \textbf{Requirement} & \textbf{Max Sec} \\
\hline
To start off, can you tell me a bit about your background? Where did you grow up, and what was it like? You can share anything about your family, your neighborhood, friends, or anything else you can think of. & Learn as much as you can about the interviewee's life experience, and their personal background. Be respectful but curious as you hear about their story. Try to get some specific and detailed experiences or memories about the interviewee's life. & 30 \\
\hline
Now I'd like to ask you about an important relationship in your life. Who is someone who has had a big impact on you? Can you tell me about your relationship with them—how you met, what they mean to you, and any important memories you've shared? & Learn about a personally meaningful relationship. Encourage storytelling and emotional depth. Ask follow-ups to explore how this relationship shaped the interviewee's identity, values, or perspective. & 30 \\
\hline
Can you tell me about the work you do now? What's your job like, and how do you feel about it day to day? & Learn about what the interviewee does for a living. Be curious but respectful as you hear about their story. Follow up and ask what they like and dislike about their job. & 45 \\
\hline
Generally, what could be done to make your work life better? You can discuss whatever you feel would make your life better, either now or in the past.  & Learn about what the interviewee thinks could be done to make their work life better. Be curious about their thoughts. Try to get some specific examples or ideas about how to improve their work life. If they need inspiration, you can give them some ideas but try not to bias them. If their answers are too brief or surface-level, probe further to understand their reasoning. You can even ask them what they would tell someone in-power like a lawmaker or employer. & 60 \\
\hline
We're now going to turn to the topic of the minimum wage. How would changes in the minimum wage (either raising or lowering it) affect you, your family, or anyone else you know personally? & Learn about how the interviewee thinks changes in the minimum wage would affect them, their family, or anyone else they know personally. Be curious about their thoughts. Make sure you ask follow up questions to get more specific on how they would be impacted. If they say they would be negatively impacted, ask why they think that. If they do not think they would be impacted, prompt them to think about different people they interact with that may be impacted. & 60 \\
\hline
What do you think is a fair minimum wage in your area? Why? & Understand the interviewee's thoughts on what a fair minimum wage is. Be curious and try to get some specific and detailed thoughts about the interviewee's thoughts on what a fair minimum wage is. For example, you can ask them to think about rent, food, and other basic necessities in their area. & 45 \\
\hline
If you earned more, what would you do with the extra money? & Learn about how the interviewee would spend extra money. You can also ask how it would make them feel to have the extra money, and what goals it would allow them to achieve. & 45 \\
\hline
Do you have any concerns about raising the minimum wage to \textbackslash{}$30 an hour? & Surface how the interviewee thinks about economic trade-offs and competing narratives. If they cannot think of any downsides, you can provide some examples, such as higher prices, less jobs, etc. & 45 \\
\hline
I'd now like to ask you about discrimination. Have you ever experienced discrimination? If so, can you tell me about it? & Learn about the interviewee's experiences with discrimination. Be curious and try to get some specific and detailed experiences or memories about the interviewee's experience with discrimination. Follow up with questions about whether they have experienced discrimination in the workplace or hiring. If they say they have never experienced discrimination, ask them if anyone they know has experienced discrimination. If they say they have not experienced discrimination nor have anyone they know has experienced discrimination, then ask them whether they think discrimination is a problem in society and why. & 60 \\
\hline
How would you feel if you knew that race or gender was a factor in a hiring decision that affected you? & Understand the interviewee's thoughts on how they would feel if they knew that race or gender was a factor in hiring decisions. Be curious and try to get some specific and detailed thoughts about the interviewee's thoughts on how they would feel if they knew that race or gender was a factor in hiring decisions. & 45 \\
\hline
Do you think race or gender should be taken into account for hiring decisions to combat gender and racial inequality? Why or why not? & Understand the interviewee's thoughts on whether race or gender should be taken into account for hiring decisions. Be curious and try to get some specific and detailed thoughts about the interviewee's thoughts on whether race or gender should be taken into account for hiring decisions. & 45 \\
\hline
We're now going to move to a new topic. Have you ever worked with or known someone at work from another country? What was your experience like? & Understand whether the interviewee has worked with or known someone from another country. If they have, ask them specifics questions about their experience working with them and what it was like. If they have not, ask them if they have friends or family who are from another country, or they themselves are from another country. If they know someone from another country, ask them about that relationship and what it was like. & 45 \\
\hline
Have you or someone close to you ever been impacted by immigration policy, especially around work or hiring? & Understand whether the interviewee has been impacted by immigration policy. If they have, ask them specifics questions about their experience and what it was like. If they have not, ask them if they have friends or family who have been impacted by immigration policy. Try to get specific experiences or memories about the interviewee's experience with immigration policy if they have been impacted. If they have not been impacted at all nor have anyone they know has been impacted, then the objective has been met. & 45 \\
\hline
Do you think it matters where someone is from when hiring for a job, as long as they’re qualified? Why or why not? & Understand the interviewee's thoughts on whether it matters where someone is from when hiring for a job, as long as they’re qualified. Try to understand the benefits and drawbacks they see. Also follow up by asking if there are any situations where nationality or immigration status should be considered. & 45 \\
\hline
How do you feel about the idea that companies should prioritize hiring local applicants over foreign applicants? & Understand the interviewee's thoughts on the idea that companies should prioritize hiring local applicants over foreign applicants. Follow up by asking them the benefits and drawbacks of this idea. & 45 \\
\hline
\end{tabular}
\caption{Interview Questions with Requirements and Maximum Time}
\label{tab:questions}
\end{table}

==> tables/topics_and_opinions.tex <==
{\footnotesize

\begin{longtable}{p{2cm}p{4cm}cccccccc}
\caption{Outcomes associated with topic learning and opinion shifts across visualization and interview modes.} \\
\toprule
\multicolumn{2}{c}{} & \multicolumn{4}{c}{\textbf{Visualization}} & \multicolumn{4}{c}{\textbf{Interview}} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10}
\textbf{Category} & \textbf{Outcome} & Coef. & 90\% CI & pval & qval & Coef. & 90\% CI & pval & qval \\
\midrule
\endfirsthead

\toprule
\multicolumn{2}{c}{} & \multicolumn{4}{c}{\textbf{Visualization}} & \multicolumn{4}{c}{\textbf{Interview}} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10}
\textbf{Category} & \textbf{Outcome} & Coef. & 90\% CI & pval & qval & Coef. & 90\% CI & pval & qval \\
\midrule
\endhead

\bottomrule
\endfoot

\multirow{3}{*}{\parbox{2cm}{Change stance (self reported)}} & Compared to before this process, my beliefs on the minimum wage issue have: & 0.19 & [-0.10, 0.49] & 0.28 & 0.28 & -0.07 & [-0.38, 0.23] & 0.68 & 0.68 \\
& Compared to before this process, my beliefs on hiring international applicants has: & 0.28 & [0.01, 0.55] & 0.09 & 0.18 & -0.10 & [-0.37, 0.18] & 0.56 & 0.68 \\
& Compared to before this process, my beliefs on whether race or gender should be used in hiring decisions have: & 0.26 & [-0.02, 0.53] & 0.12 & 0.18 & -0.20 & [-0.48, 0.08] & 0.23 & 0.68 \\

\multirow{3}{*}{\parbox{2cm}{Learning (foreign vs. domestic workers)}} & \textbf{Compared to before, I feel more informed about why people may have different beliefs on hiring locals over international applicants.} & 2.05*** & [1.42, 2.68] & 0.00 & 0.00 & 0.80** & [0.16, 1.45] & 0.04 & 0.05 \\
& \textbf{I feel more informed about the topic of hiring locals over international applicants} & 1.85*** & [1.20, 2.50] & 0.00 & 0.00 & 1.02** & [0.35, 1.68] & 0.01 & 0.04 \\
& \textbf{This exercise has taught me something about the topic of hiring locals over international applicants.} & 1.86*** & [1.20, 2.52] & 0.00 & 0.00 & 0.82** & [0.14, 1.49] & 0.05 & 0.05 \\

\multirow{3}{*}{\parbox{2cm}{Learning (min. wage)}} & \textbf{Compared to before, I feel more informed about why people may have different beliefs on raising the minimum wage.} & 1.84*** & [1.19, 2.49] & 0.00 & 0.00 & 1.13** & [0.46, 1.79] & 0.01 & 0.02 \\
& \textbf{I feel more informed about the topic of raising the minimum wage.} & 1.71*** & [1.05, 2.38] & 0.00 & 0.00 & 0.80* & [0.12, 1.48] & 0.05 & 0.05 \\
& \textbf{This exercise has taught me something about raising the minimum wage.} & 1.62*** & [0.96, 2.27] & 0.00 & 0.00 & 0.80* & [0.13, 1.47] & 0.05 & 0.05 \\

\multirow{3}{*}{\parbox{2cm}{Learning (race \& gender in hiring)}} & \textbf{Compared to before, I feel more informed about why people may have different beliefs about the topic of using race and gender in hiring.} & 1.88*** & [1.25, 2.52] & 0.00 & 0.00 & 0.98** & [0.33, 1.63] & 0.01 & 0.02 \\
& \textbf{I feel more informed about the topic of using race and gender in hiring decisions.} & 1.97*** & [1.32, 2.62] & 0.00 & 0.00 & 1.13** & [0.46, 1.79] & 0.01 & 0.02 \\
& \textbf{This exercise has taught me something about the topic of using race and gender in hiring decisions.} & 1.55*** & [0.87, 2.22] & 0.00 & 0.00 & 0.79* & [0.10, 1.48] & 0.06 & 0.06 \\

\multirow{3}{*}{\parbox{2cm}{Stance certainty (foreign vs. domestic workers)}} & I hold strong beliefs about whether companies should prioritize locals over international applicants. & -0.36 & [-0.80, 0.08] & 0.17 & 0.26 & 0.08 & [-0.37, 0.53] & 0.77 & 0.82 \\
& I feel certain that my stance on whether companies should prioritize local applicants over international ones is the right one. & -0.31 & [-0.75, 0.14] & 0.26 & 0.26 & -0.12 & [-0.58, 0.34] & 0.66 & 0.82 \\
& I don't think there are good arguments against my position on whether to prioritize locals over international applicants. & -0.72 & [-1.35, -0.10] & 0.06 & 0.18 & -0.09 & [-0.73, 0.56] & 0.82 & 0.82 \\

\multirow{3}{*}{\parbox{2cm}{Stance certainty (min. wage)}} & I hold strong beliefs about whether the federal minimum wage should be raised. & 0.15 & [-0.28, 0.58] & 0.58 & 0.86 & 0.31 & [-0.13, 0.75] & 0.24 & 0.73 \\
& I feel certain that my stance on the federal minimum wage is the right one. & -0.04 & [-0.52, 0.44] & 0.89 & 0.89 & 0.00 & [-0.49, 0.50] & 0.99 & 0.99 \\
& I don't think there are good arguments against my position on whether to raise the federal minimum wage. & -0.34 & [-0.96, 0.28] & 0.37 & 0.86 & -0.24 & [-0.88, 0.39] & 0.53 & 0.79 \\

\multirow{3}{*}{\parbox{2cm}{Stance certainty (race \& gender in hiring)}} & \textbf{I hold strong beliefs about whether race and gender should be used in hiring decisions.} & 0.07 & [-0.36, 0.51] & 0.78 & 0.80 & 0.63* & [0.18, 1.07] & 0.02 & 0.07 \\
& I feel certain that I hold the correct belief on whether race and gender should be used in hiring decisions. & -0.07 & [-0.54, 0.40] & 0.80 & 0.80 & 0.52 & [0.04, 1.00] & 0.08 & 0.12 \\
& I don't think there are good arguments against my position on whether race and gender should be used in hiring decisions. & -0.22 & [-0.83, 0.38] & 0.54 & 0.80 & 0.05 & [-0.57, 0.67] & 0.90 & 0.90 \\

\multirow{3}{*}{\parbox{2cm}{Topic Stance}} & How much do you agree with the following statement? "The federal minimum wage should be raised to \$30 an hour." & 0.01 & [-0.47, 0.49] & 0.97 & 0.97 & -0.23 & [-0.73, 0.27] & 0.44 & 0.80 \\
& How much do you agree with the following statement? "Companies should strongly prioritize hiring domestically before considering foreign applicants." & 0.39 & [-0.22, 1.00] & 0.29 & 0.85 & 0.10 & [-0.53, 0.72] & 0.80 & 0.80 \\
& How much do you agree with the following statement? "Race and gender should be used in hiring decisions to combat inequality in the workplace." & 0.20 & [-0.38, 0.79] & 0.57 & 0.85 & -0.18 & [-0.78, 0.42] & 0.62 & 0.80 \\

\end{longtable}
}


==> tables/treatments.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{>{\centering\arraybackslash}p{0.15\linewidth}p{0.75\linewidth}p{0.06\linewidth}}
\toprule
\textbf{Condition} & \textbf{Description} & \textbf{n} \\
\midrule
A & Took AI interview \textbf{AND} saw voting visualization & 42 \\
B & Took AI interview but did \textbf{NOT} see voting visualization & 48 \\
C & No AI interview but saw voting visualization & 44 \\
D & No AI interview and did \textbf{NOT} see voting visualization & 47 \\
\bottomrule
\end{tabular}
\caption{Treatment groups, descriptions, and participant counts [ADD NEW COLUMN WITH INTERFACE FEATURES HERE].}
\label{tab:treatment_groups}
\end{table}

